Mission-Critical Public Safety Networking: An Intent-Driven Service Orchestration Perspective

Intent-based networking (IBN) provides a promising approach for managing networks and orchestrating services in beyond 5G (B5G) deployments using modern service-based architectures. Public safety (PS) services form the basis of keeping society functional, owing to the responsiveness and availability throughout the network. The provisioning of these services requires efficient and agile network management techniques with low-overhead and embedded intelligence. IBN incorporates the service subscribers in a model-driven approach to provision different user-centric services. However, it requires domain-specific and contextual processing of intents for abstracted management of network functions. This work proposes an intent definition for PS and mission critical (MC) services in beyond B5G networks, as well as a processing and orchestration architecture on top of MC push-to-talk (PTT) use case. The simulation results show that MC PTT services adhere to the key performance indicators of access time and mouth-to-ear latency bounded by approximately 250 and 150 milliseconds, respectively, with an additional overhead experienced during the intent processing in the range of 20- 40 milliseconds. This validates the premise of IBN in providing flexible and scalable management and service orchestration solution for PS next generation networks.

==> Resources/Others/_1-Plan.tex <==

% \begin{figure}[ht!]
% \begin{center}
%     \includegraphics[width=0.9\textwidth]{Resources/Images/icc-ibn-model.png}
% \end{center}
% \caption{IBN Orchestration Model}
% \label{image: organization}
% \end{figure}

\section*{Organization and Planning}
A brief summary of sections and their contents is as follows:
\begin{enumerate}
    \item Section-I: Introduction
    \begin{itemize}
        \item Critical nature of mission critical services and public safety networks
        \item IBN as a key enabler for network automation and user centric service design, orchestration
        \item State of the art and prevalent issues in PSC and MC services in terms of known metrics
        \item Problem statement, description and discussion with related studies for IBN and PSC use cases
        \item A description of contributions from proposed model to experiments
        \item Paper structure and organization
    \end{itemize}
    \item Section-II: System Model
    \begin{itemize}
        \item Description of the component modules for provisioning MCPTT services
        \item Intent model for acquiring, describing, translation and mapping user intention towards network and device level resource provisioning and allocation strategies
        \item A discussion on the relation between IBN and MCPTT services for justification and rationale behind user involvement and automation in network orchestration
        \item Validation model for the performance evaluation of the MCPTT metrics in a PSC environment
    \end{itemize} 
    \item Section-III: Performance Evaluation

\end{enumerate}


==> Resources/Others/misc.tex <==


